Towards Aligned Layout Generation via Diffusion Model with Aesthetic Constraints

Controllable layout generation refers to the process of creating a plausible visual arrangement of elements within a graphic design (e.g., document and web designs) with constraints representing design intentions. Although recent diffusion-based models have achieved state-of-the-art FID scores, they tend to exhibit more pronounced misalignment compared to earlier transformer-based models. In this work, we propose the $\textbf{LA}$yout $\textbf{C}$onstraint diffusion mod$\textbf{E}$l (LACE), a unified model to handle a broad range of layout generation tasks, such as arranging elements with specified attributes and refining or completing a coarse layout design. The model is based on continuous diffusion models. Compared with existing methods that use discrete diffusion models, continuous state-space design can enable the incorporation of differentiable aesthetic constraint functions in training. For conditional generation, we introduce conditions via masked input. Extensive experiment results show that LACE produces high-quality layouts and outperforms existing state-of-the-art baselines.

==> section/Background.tex <==
\section{Background}
Diffusion models \cite{ho2020denoising} are generative models characterized by a forward and reverse Markov process. 
In the forward process, a continuous valued data-point $\mathbf{x}_0$ is gradually corrupted to intermediate noisy latents $\mathbf{x}_{1:T}$, which converges to a random variable of the standard multi-variant Gaussian distribution $\mathcal{N}(0, \mathbf{I})$ after $T$ steps. The transition steps between adjacent intermediate predictions is modeled as Gaussian distributions, $q(\mathbf{x}_{t} | \mathbf{x}_{t-1}) = \mathcal{N}(\mathbf{x}_t; \sqrt{1-\beta_t}\mathbf{x}_{t-1}, \beta_t \mathbf{I})$, with a variance schedule $\beta_1, \cdots, \beta_T$. The forward process admits a closed-form sampling distribution, $q(\mathbf{x}_{t} |\mathbf{x}_{0}) = \mathcal{N}(\mathbf{x}_{t}; \sqrt{\bar{\alpha}_t} \mathbf{x}_{0}, (1 - \bar{\alpha}_t)\mathbf{I}$ at arbitrary timestep $t$, where $\bar{\alpha}_t = \prod_{s=1}^t \alpha_s$ and $\alpha_t = (1 - \beta_t)$.

In the reverse (generative) process, the data $\mathbf{x}_0$ is reconstructed gradually by sampling from a series of estimated transition distributions $p_{\theta}(\mathbf{x}_{t-1} | \mathbf{x}_{t})$ start from a standard Gaussian random variable $X_T \sim \mathcal{N}(0, \mathbf{I})$. The transition distributions are learned by optimizing the evidence lower bound consists of a series of KL-divergence:
\begin{equation}
\label{eq:loss}
\mathbb{E}_q \left [ D_{\text{KL}} \left ( q(\mathbf{x}_{T} | \mathbf{x}_0) || p(\mathbf{x}_{T}) \right ) + \sum_{t>1}^{T} D_{\text{KL}} \left ( q(\mathbf{x}_{t-1} | \mathbf{x}_t, \mathbf{x}_0) || p_{\theta}(\mathbf{x}_{t-1} | \mathbf{x}_t) \right ) -\log p_{\theta}(\mathbf{x}_0 | \mathbf{x}_1) \right ].
\end{equation}

Since the posterior distributions $q(\mathbf{x}_{t-1} | \mathbf{x}_t, \mathbf{x}_0)$ are also Gaussian for an infinitesimal variance $\beta_t$ \cite{feller2015theory} and can be approximated by $\mathbf{x}_0$-parameterization \cite{song2020denoising} as:
\begin{align}
    & q(\mathbf{x}_{t-1} | \mathbf{x}_t, \mathbf{x}_0) = \mathcal{N}(\mathbf{x}_{t-1}; \Tilde{\boldsymbol \mu} (\mathbf{x}_{t}, t), \Tilde{\beta}_t \mathbf{I})\\
    \text{where} \quad & \Tilde{\boldsymbol \mu} (\mathbf{x}_{t}, t) = \frac{1}{\sqrt{\alpha_t}} \left (\mathbf{x}_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} {\boldsymbol{\epsilon}} \right ), \; {\boldsymbol{\epsilon}} \sim \mathcal{N}(0, \mathbf{I}) \;\; \text{and} \;\; \Tilde{\beta}_t = \frac{1 - \bar{\alpha}_{t-1}}{1 - \bar{\alpha}_t} \beta_t,
\end{align}
the transition distributions could be estimated as a Gaussian with a mean:
\begin{equation}
    \boldsymbol{\mu_{\theta}}(\mathbf{x}_t, t) = \frac{1}{\sqrt{\alpha_t}} \left (\mathbf{x}_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} {\boldsymbol{\epsilon}}_{\theta}(\mathbf{x}_t, t) \right ),
\end{equation}
where ${\boldsymbol{\epsilon}}_{\theta}$ is a function approximator and is usually trained using a simplified objective: 
\begin{equation}
\mathcal{L}_{\text{simple}} = ||{\boldsymbol \epsilon} - \Tilde{\boldsymbol \epsilon}_{\theta} (\sqrt{\bar{\alpha}_t} \mathbf{x}_0 + \sqrt{1 - \bar{\alpha}_t} {\boldsymbol \epsilon}, t)||^2,
\end{equation}
where ${\boldsymbol{\epsilon}} \sim \mathcal{N}(0, \mathbf{I})$.

